Prompt Performance Prediction for Image Generation

The ability to predict the performance of a query before results are returned has been a longstanding challenge in Information Retrieval (IR) systems. Inspired by this task, we introduce, in this paper, a novel task called "Prompt Performance Prediction" (PPP) that aims to predict the performance of a prompt, before obtaining the actual generated images. We demonstrate the plausibility of our task by measuring the correlation coefficient between predicted and actual performance scores across: three datasets containing pairs of prompts and generated images AND three art domain datasets of real images and real user appreciation ratings. Our results show promising performance prediction capabilities, suggesting potential applications for optimizing user prompts.

==> tables/paintings_datasets.tex <==

\begin{table*}
\centering
\resizebox{1.98\columnwidth}{!}{
\begin{tabular}{|l||c|c|c|}
\hline
Dataset                   & JenAesthetics \cite{amirshahi2015jenaesthetics}    & (Sidhu, et al.) \cite{sidhu2018prediction} & VAPS-999 \cite{fekete2022vienna}   \\ \hline \hline
Total pictures $|$ Missing            & 1628  $|$  65   (3.99\%)     & 480   $|$  6 (1.25\%)                                               & 999   $|$  3  (0.30\%)                                             \\ \hline
%Missing / corrupted pictures            & 65   (3,99\%)                                                             & 6 (1,25\%)                                                & 3  (0,30\%)                                               \\ \hline
Total participants        & 134                                                                 & 598                                                         & 120 (60 M, 60 F)                                    \\ \hline
%Nb. observers per image    & 19 - 21                                                             & \textgreater{}= 40                                          & 20 (120 for 55 images)                              \\ \hline
Diversity of participants & \makecell{15 countries \\ (109 from Germany)}                                     &          \makecell{University of Calgary \\ undergraduates}                                                   & \makecell{ University of Vienna students \\ 60 M, 60 F} \\ \hline %(114 studied psychology)}                                  \\ \hline
Styles covered            &  Renaissance $\xrightarrow{}$ Expressionism                                   & \makecell{Half abstract \\ half representationnal}                       & 1434 $-$ 2012                                         \\ \hline
Community                 & Computer Vision                                                     & Psychology                                                  & Psychology \& Art                                   \\ \hline
Appreciation features     & \makecell{Aesthetic, Beauty, \\ Liking Color / Composition / Content} & \makecell{Meaningfulness, Complexity \\ Emotion, Beauty, Liking}                                       & Cognitive, Affective, Liking                      \\
\hline
\end{tabular}}
\caption{The datasets of paintings used in the experiments detailed in Section \ref{sec:experiments}, each associated with liking ratings and appreciation. These datasets cover a wide range of styles and epochs of painting, with diverse representation of communities judging the paintings.}
    \label{tab:paintings_datasets}
\end{table*}



==> tables/paintings_scores.tex <==

\begin{table}
    \centering
    \resizebox{0.99\columnwidth}{!}{
    \begin{tabular}{|l|c|c|c|}
        \hline
        Method & VAPS-999    &  Sidhu & JenAesthetics \\ %\cite{fekete2022vienna}  \\ %Pearson $r$ &  \\
        \hline \hline
        LAION Aesthetic Predictor & \textbf{0.2232}  & \textbf{0.2938} & \textbf{0.1635} \\ \hline 
        %Male/Female correlation   & \textbf{0.6067}  & $-$ & $-$ \\ \hline 
        \hline
        Text-based : \textcolor{applegreen}{Valence} & 0.4025 & 0.5980 & $-$ \\ \hline
        Text-based : \textcolor{babyblueeyes}{Description} & 0.4401  & 0.3689 & 0.5452 \\ \hline
        Text-based : \textcolor{candypink}{Painter + epoch} & 0.5471  & 0.4185 & 0.4826 \\ \hline
        \makecell[l]{Text-based : \textcolor{babyblueeyes}{Description} \\ + \textcolor{candypink}{painter + epoch}} & 0.5989  & 0.4955 & \textbf{0.5805} \\ \hline
         Generated images & 0.5888 & $-$  & $-$ \\ \hline
        \makecell[l]{Text-based : \textcolor{babyblueeyes}{Description} \\ + \textcolor{candypink}{painter + epoch}  +  \textcolor{applegreen}{valence}} & \textbf{0.6581} & \textbf{0.6204} & $-$ \\ \hline\hline
        Image-based  features  & \textbf{0.7269} & \textbf{0.7939} & \textbf{0.7366} \\ \hline
    \end{tabular}}
    \caption{Pearson correlation results between the appreciation ground truth and appreciation predictions of the paintings of each of the three datasets \cite{amirshahi2015jenaesthetics,fekete2022vienna,sidhu2018prediction} of our study (all $p$-value $< 0.01$), made using the Laion Aesthetic Predictor \cite{laion} pretrained on photography and natural images (top),  our proposed text-based approach with varying degrees of information for prediction using text-based features of paintings (middle), and an image prediction model with image-based features of the paintings (bottom). The text-based and image-based approach use the same CLIP ViT-L-14 encoder \cite{radford2021learning} coupled with a linear layer for regression.}
    \label{tab:scores_vit14}
    %\vspace{-3pt}
\end{table}




==> tables/pipo_grid_search_different_text_extractors_rbf.tex <==
\begin{table}[!hbp]
\centering
\caption{Best mean\_test\_pearsonr by ebds\_name for RBF kernel}
\resizebox{1.99\columnwidth}{!}{
\begin{tabular}{llcccccccc}
\toprule
                 & ebds\_name &    bart &    gpt2 & bloom560m & sentence-t5-xl & sentence-t5-base & sentence-t5-large & clip\_ViT-B-32\_prompt & clip\_ViT-L-14\_prompt \\
dataset\_name & scores\_name &         &         &           &                &                  &                   &                      &                      \\
\midrule
Dall-E 2 & ResMem &  0.5961 &  0.5371 &    0.5434 &         0.6449 &           0.6303 &            0.6385 &               0.6715 &               0.6724 \\
                 & SAMPNet &  0.5125 &  0.4498 &     0.452 &         0.5729 &           0.5559 &             0.568 &               0.6056 &                0.609 \\
                 & ViTMem &  0.6761 &   0.603 &    0.6133 &         0.7301 &           0.7123 &            0.7247 &               0.7546 &               0.7551 \\
                 & clip\_ViT-B-32\_aesthetic &  0.5751 &  0.4919 &    0.4748 &         0.6391 &           0.6303 &            0.6384 &               0.6713 &               0.6733 \\
                 & clip\_ViT-L-14\_aesthetic &  0.5782 &   0.502 &    0.4923 &         0.6407 &           0.6353 &            0.6417 &               0.6693 &               0.6721 \\
                 & improved\_aesthetic\_predictor &  0.6084 &  0.5261 &    0.5156 &         0.6622 &           0.6578 &             0.665 &               0.6866 &               0.6932 \\
MidJourney & ResMem &  0.7592 &  0.6823 &    0.6779 &         0.8171 &           0.8049 &            0.8141 &                0.864 &               0.8507 \\
                 & SAMPNet &  0.6907 &  0.6017 &    0.6038 &         0.7638 &           0.7503 &            0.7582 &               0.8289 &                0.813 \\
                 & ViTMem &  0.7859 &  0.7031 &    0.6995 &         0.8426 &           0.8303 &            0.8391 &               0.8899 &               0.8766 \\
                 & clip\_ViT-B-32\_aesthetic &  0.6706 &  0.5525 &    0.5508 &         0.7464 &           0.7354 &             0.743 &               0.8148 &               0.8008 \\
                 & clip\_ViT-L-14\_aesthetic &  0.6658 &  0.5562 &    0.5537 &         0.7339 &           0.7259 &            0.7334 &               0.7927 &               0.7841 \\
                 & improved\_aesthetic\_predictor &  0.7278 &  0.5935 &    0.5988 &          0.773 &           0.7594 &            0.7693 &               0.8279 &               0.8192 \\
Stable Diffusion & ResMem &  0.6319 &  0.5538 &    0.5544 &         0.7037 &           0.6814 &            0.6995 &               0.7581 &                0.774 \\
                 & SAMPNet &  0.5647 &    0.47 &    0.4727 &         0.6585 &           0.6332 &            0.6551 &                0.728 &               0.7448 \\
                 & ViTMem &  0.6959 &  0.5944 &    0.6011 &         0.7618 &           0.7434 &            0.7617 &               0.8102 &                0.824 \\
                 & clip\_ViT-B-32\_aesthetic &  0.5619 &  0.4586 &    0.4593 &         0.6299 &           0.6168 &            0.6305 &               0.6951 &                0.708 \\
                 & clip\_ViT-L-14\_aesthetic &  0.5884 &  0.4901 &     0.494 &         0.6356 &           0.6223 &            0.6362 &               0.7004 &               0.7158 \\
                 & improved\_aesthetic\_predictor &  0.7482 &  0.6649 &    0.6784 &         0.7789 &           0.7661 &            0.7794 &               0.8267 &               0.8381 \\
\bottomrule
\end{tabular}
}
\label{tab:rbf}
\end{table}

